BELLATREX: Building Explanations through a LocaLly AccuraTe Rule EXtractor

Tree-ensemble algorithms, such as random forest, are effective machine learning methods popular for their flexibility, high performance, and robustness to overfitting. However, since multiple learners are combined, they are not as interpretable as a single decision tree. In this work we propose a novel method that is Building Explanations through a LocalLy AccuraTe Rule EXtractor (Bellatrex), and is able to explain the forest prediction for a given test instance with only a few diverse rules. Starting from the decision trees generated by a random forest, our method 1) pre-selects a subset of the rules used to make the prediction, 2) creates a vector representation of such rules, 3) projects them to a low-dimensional space, 4) clusters such representations to pick a rule from each cluster to explain the instance prediction. We test the effectiveness of Bellatrex on 89 real-world datasets and we demonstrate the validity of our method for binary classification, regression, multi-label classification and time-to-event tasks. To the best of our knowledge, it is the first time that an interpretability toolbox can handle all these tasks within the same framework. We also show that our extracted surrogate model can approximate the performance of the corresponding ensemble model in all considered tasks, while selecting only few trees from the whole forest. We also show that our proposed approach substantially outperforms other explainable methods in terms of predictive performance.

==> biblio_full.tex <==

@article{Nori2019,
abstract = {InterpretML is an open-source Python package which exposes machine learning interpretability algorithms to practitioners and researchers. InterpretML exposes two types of interpretability - glassbox models, which are machine learning models designed for interpretability (ex: linear models, rule lists, generalized additive models), and blackbox explainability techniques for explaining existing systems (ex: Partial Dependence, LIME). The package enables practitioners to easily compare interpretability algorithms by exposing multiple methods under a unified API, and by having a built-in, extensible visualization platform. InterpretML also includes the first implementation of the Explainable Boosting Machine, a powerful, interpretable, glassbox model that can be as accurate as many blackbox models. The MIT licensed source code can be downloaded from github.com/microsoft/interpret.},
archivePrefix = {arXiv},
arxivId = {1909.09223},
author = {Nori, Harsha and Jenkins, Samuel and Koch, Paul and Caruana, Rich},
eprint = {1909.09223},
keywords = {Blackbox,Explainable Boosting Machine,Glassbox,Interpretability},
month = {sep},
title = {{InterpretML: A Unified Framework for Machine Learning Interpretability}},
url = {http://arxiv.org/abs/1909.09223},
year = {2019}
}

@article{Guidotti2018,
abstract = {In recent years, many accurate decision support systems have been constructed as black boxes, that is as systems that hide their internal logic to the user. This lack of explanation constitutes both a practical and an ethical issue. The literature reports many approaches aimed at overcoming this crucial weakness, sometimes at the cost of sacrificing accuracy for interpretability. The applications in which black box decision systems can be used are various, and each approach is typically developed to provide a solution for a specific problem and, as a consequence, it explicitly or implicitly delineates its own definition of interpretability and explanation. The aim of this article is to provide a classification of the main problems addressed in the literature with respect to the notion of explanation and the type of black box system. Given a problem definition, a black box type, and a desired explanation, this survey should help the researcher to find the proposals more useful for his own work. The proposed classification of approaches to open black box models should also be useful for putting the many research open questions in perspective.},
author = {Guidotti, Riccardo and Monreale, Anna and Ruggieri, Salvatore and Turini, Franco and Giannotti, Fosca and Pedreschi, Dino},
doi = {10.1145/3236009},
issn = {15577341},
journal = {ACM Computing Surveys},
keywords = {Explanations,Interpretability,Open The Black Box,Transparent Models},
mendeley-groups = {Biblio for ECML-2022},
number = {5},
title = {{A survey of methods for explaining black box models}},
volume = {51},
year = {2018}
}


@article{Haddouchi2019,
abstract = {Interpretability of highly performant Machine Learning [ML] methods, such as Random Forest [RF], is a key tool that attracts a great interest in datamining research. In the state of the art, RF is well-known as an efficient ensemble learning (in terms of predictive accuracy, flexibility and straightforwardness). Moreover, it is recognized as an intuitive and intelligible approach regarding to its building process. However it is also regarded as a Black Box model because of its hundreds of deep decision trees. This can be crucial for several fields of study, such as healthcare, biology and security, where the lack of interpretability could be a real disadvantage. Indeed, the interpretability of the RF models is, generally, necessary in such fields of applications because of different motivations. In fact, the more the ML users grasp what is going on inside a ML system (process and resulting model), the more they can trust it and take actions based on the knowledge extracted from it. Furthermore, ML models are increasingly constrained by new laws that require regulation and interpretation of the knowledge they provide.Several papers have tackled the interpretation of RF resulting models. It had been associated with different aspects depending on the specificity of the issue studied as well as the users concerned with explanations. Therefore, this paper aims to provide a survey of tools and methods used in literature in order to uncover insights in the RF resulting models. These tools are classified depending on different aspects characterizing the interpretability. This should guide, in practice, in the choice of the most useful tools for interpretation and deep analysis of the RF model depending on the interpretability aspect sought. This should also be valuable for researchers who aim to focus their work on the interpretability of RF, or ML in general.},
author = {Haddouchi, Maissae and Berrado, Abdelaziz},
doi = {10.1109/ICSSD47982.2019.9002770},
isbn = {9781728143682},
journal = {ICSSD 2019 - International Conference on Smart Systems and Data Science},
keywords = {Interpretability,Random Forest,Tree Ensemble,review,survey},
mendeley-groups = {Interpretable TreeEnsembles,About X-AI,Biblio for ECML-2022},
title = {{A survey of methods and tools used for interpreting Random Forest}},
year = {2019}
}


@techreport{Arya2020,
abstract = {As artificial intelligence algorithms make further inroads in high-stakes societal applications, there are increasing calls from multiple stakeholders for these algorithms to explain their outputs. To make matters more challenging, different personas of consumers of explanations have different requirements for explanations. Toward addressing these needs, we introduce AI Explainability 360, an open-source Python toolkit featuring ten diverse and state-of-the-art explainability methods and two evaluation metrics (http://aix360.mybluemix.net). Equally important, we provide a taxonomy to help entities requiring explanations to navigate the space of interpretation and explanation methods, not only those in the toolkit but also in the broader literature on explain-ability. For data scientists and other users of the toolkit, we have implemented an extensible software architecture that organizes methods according to their place in the AI modeling pipeline. The toolkit is not only the software, but also guidance material, tutorials, and an interactive web demo to introduce AI explainability to different audiences. Together, our toolkit and taxonomy can help identify gaps where more explainability methods are needed and provide a platform to incorporate them as they are developed.},
author = {Arya, Vijay and Bellamy, Rachel K E and Chen, Pin-Yu and Dhurandhar, Amit and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Liao, Q Vera and Luss, Ronny and Mourad, Sami and Pedemonte, Pablo and Raghavendra, Ramya and Richards, John T and Sattigeri, Prasanna and Shanmugam, Karthikeyan and Singh, Moninder and Varshney, Kush R and Wei, Dennis and Zhang, Yunfeng},

booktitle = {Journal of Machine Learning Research},
keywords = {explainability,interpretability,open source,taxonomy,transparency},
pages = {1--6},
title = {{AI Explainability 360: An Extensible Toolkit for Understanding Data and Machine Learning Models}},
url = {http://aix360.mybluemix.net},
volume = {21},
year = {2020}
}

@article{Vidal2020,
abstract = {The use of machine learning algorithms in finance, medicine, and criminal justice can deeply impact human lives. As a consequence, research into interpretable machine learning has rapidly grown in an attempt to better control and fix possible sources of mistakes and biases. Tree ensembles offer a good prediction quality in various domains, but the concurrent use of multiple trees reduces the interpretability of the ensemble. Against this background, we study born-again tree ensembles, i.e., the process of constructing a single decision tree of minimum size that reproduces the exact same behavior as a given tree ensemble. To find such a tree, we develop a dynamic-programming based algorithm that exploits sophisticated pruning and bounding rules to reduce the number of recursive calls. This algorithm generates optimal born-again trees for many datasets of practical interest, leading to classifiers which are typically simpler and more interpretable without any other form of compromise.},

archivePrefix = {arXiv},
arxivId = {2003.11132},
author = {Vidal, Thibaut and Pacheco, Toni and Schiffer, Maximilian},
eprint = {2003.11132},
journal = {arXiv},
number = {D},
title = {{Born-again Tree Ensembles}},
year = {2020}
}
@article{Kaur2020,
abstract = {Machine learning (ML) models are now routinely deployed in domains ranging from criminal justice to healthcare. With this newfound ubiquity, ML has moved beyond academia and grown into an engineering discipline. To that end, interpretabil-ity tools have been designed to help data scientists and machine learning practitioners better understand how ML models work. However, there has been little evaluation of the extent to which these tools achieve this goal. We study data scien-tists' use of two existing interpretability tools, the InterpretML implementation of GAMs and the SHAP Python package. We conduct a contextual inquiry (N=11) and a survey (N=197) of data scientists to observe how they use interpretability tools to uncover common issues that arise when building and evaluating ML models. Our results indicate that data scientists over-trust and misuse interpretability tools. Furthermore, few of our participants were able to accurately describe the visual-izations output by these tools. We highlight qualitative themes for data scientists' mental models of interpretability tools. We conclude with implications for researchers and tool designers, and contextualize our findings in the social science literature.},
author = {Kaur, Harmanpreet and Nori, Harsha and Jenkins, Samuel and Caruana, Rich and Wallach, Hanna and {Wortman Vaughan}, Jennifer},
doi = {10.1145/3313831.3376219},
isbn = {9781450367080},
journal = {dl.acm.org},
keywords = {interpretability,machine learning,user-centric evaluation},
month = {apr},
publisher = {Association for Computing Machinery},
title = {{Interpreting Interpretability: Understanding Data Scientists' Use of Interpretability Tools for Machine Learning}},
url = {http://dx.doi.org/10.1145/3313831.3376219},
year = {2020}
}

@article{RuleCOSI+,
author = {Obregon, Josue and Jung, Jae-Yoon},
doi = {10.1016/j.inffus.2022.08.021},
issn = {15662535},
journal = {Information Fusion},
mendeley-groups = {Biblio for ECML-2022,About X-AI},
month = {aug},
publisher = {Elsevier},
title = {{RuleCOSI+: Rule extraction for interpreting classification tree ensembles}},
url = {https://linkinghub.elsevier.com/retrieve/pii/S1566253522001129},
year = {2022}
}

@article{Hoffman2018,
title={Metrics for explainable AI: Challenges and prospects},
author={Hoffman, Robert R and Mueller, Shane T and Klein, Gary and Litman, Jordan},
journal={arXiv preprint arXiv:1812.04608},
url = {http://arxiv.org/abs/1812.04608},
year = {2018}
}


@article{Doshi-Velez-2017,
  title={Towards a rigorous science of interpretable machine learning},
  author={Doshi-Velez, Finale and Kim, Been},
  journal={arXiv preprint arXiv:1702.08608},
  year={2017}
}

@article{RuleFit,
  title={Predictive learning via rule ensembles},
  author={Friedman, Jerome H and Popescu, Bogdan E},
  journal={The annals of applied statistics},
  pages={916--954},
  year={2008},
  publisher={JSTOR}
}

@article{ExtraTrees,
  title={Extremely randomized trees},
  author={Geurts, Pierre and Ernst, Damien and Wehenkel, Louis},
  journal={Machine learning},
  volume={63},
  number={1},
  pages={3--42},
  year={2006},
  publisher={Springer}
}


@article{Biau2016,
abstract = {The random forest algorithm, proposed by L. Breiman in 2001, has been extremely successful as a general-purpose classification and regression method. The approach, which combines several randomized decision trees and aggregates their predictions by averaging, has shown excellent performance in settings where the number of variables is much larger than the number of observations. Moreover, it is versatile enough to be applied to large-scale problems, is easily adapted to various ad hoc learning tasks, and returns measures of variable importance. The present article reviews the most recent theoretical and methodological developments for random forests. Emphasis is placed on the mathematical forces driving the algorithm, with special attention given to the selection of parameters, the resampling mechanism, and variable importance measures. This review is intended to provide non-experts easy access to the main ideas.},
archivePrefix = {arXiv},
arxivId = {1511.05741},
author = {Biau, G{\'{e}}rard and Scornet, Erwan},
doi = {10.1007/s11749-016-0481-7},
eprint = {1511.05741},
issn = {11330686},
journal = {Test},
keywords = {Parameter tuning,Random forests,Randomization,Resampling,Variable importance},
month = {jun},
number = {2},
pages = {197--227},
publisher = {Springer New York LLC},
title = {{A random forest guided tour}},
url = {www.kaggle.com/c/dsg-hackathon},
volume = {25},
year = {2016}
}

@article{Pedregosa2011,
  title={Scikit-learn: Machine learning in Python},
  author={Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and others},
  journal={the Journal of machine Learning research},
  volume={12},
  pages={2825--2830},
  year={2011},
  publisher={JMLR. org}
}


@misc{Turkson2021,
author = {Turkson, Anthony Joe and Ayiah-Mensah, Francis and Nimoh, Vivian},
booktitle = {International Journal of Mathematics and Mathematical Sciences},
doi = {10.1155/2021/9307475},
issn = {16870425},
publisher = {Hindawi Limited},
title = {{Handling Censoring and Censored Data in Survival Analysis: A Standalone Systematic Literature Review}},
volume = {2021},
year = {2021}
}

@article{Tan2016,
archivePrefix = {arXiv},
arxivId = {1611.07115},
author = {Tan, Sarah and Soloviev, Matvey and Hooker, Giles and Wells, Martin T.},
eprint = {1611.07115},
number = {1},
title = {{Tree Space Prototypes: Another Look at Making Tree Ensembles Interpretable}},
url = {http://arxiv.org/abs/1611.07115},
year = {2016}
}
@article{Sies2020,
abstract = {Often tree-based accounts of statistical learning problems yield multiple decision trees which together constitute a forest. Reasons for this include examining tree instability, improving prediction accuracy, accounting for missingness in the data, and taking into account multiple outcome variables. A key disadvantage of forests, unlike individual decision trees, is their lack of transparency. Hence, an obvious challenge is whether it is possible to recover some of the insightfulness of individual trees from a forest. In this paper, we will propose a conceptual framework and methodology to do so by reducing forests into one or a small number of summary trees, which may be used to gain insight into the central tendency as well as the heterogeneity of the forest. This is done by clustering the trees in the forest based on similarities between them. By means of simulated data, we will demonstrate how and why different similarity types in the proposed methodology may lead to markedly different conclusions, and explain when and why certain approaches may be recommended over other ones. We will finally illustrate the methodology with an empirical data set on the prediction of cocaine use on the basis of personality characteristics.},


author = {Sies, Aniek and {Van Mechelen}, Iven},
doi = {10.1007/s00357-019-09350-4},
issn = {14321343},
journal = {Journal of Classification},
keywords = {Bagging,Classification trees,Clustering,Ensemble methods,Statistical learning},
publisher = {Journal of Classification},
title = {{C443: a Methodology to See a Forest for the Trees}},
volume = {1},
year = {2020}
}

@article{Molnar2020,
abstract = {We present a brief history of the field of interpretable machine learning (IML), give an overview of state-of-the-art interpretation methods and discuss challenges. Research in IML has boomed in recent years. As young as the field is, it has over 200 years old roots in regression modeling and rule-based machine learning, starting in the 1960s. Recently, many new IML methods have been proposed, many of them model-agnostic, but also interpretation techniques specific to deep learning and tree-based ensembles. IML methods either directly analyze model components, study sensitivity to input perturbations, or analyze local or global surrogate approximations of the ML model. The field approaches a state of readiness and stability, with many methods not only proposed in research, but also implemented in open-source software. But many important challenges remain for IML, such as dealing with dependent features, causal interpretation, and uncertainty estimation, which need to be resolved for its successful application to scientific problems. A further challenge is a missing rigorous definition of interpretability, which is accepted by the community. To address the challenges and advance the field, we urge to recall our roots of interpretable, data-driven modeling in statistics and (rule-based) ML, but also to consider other areas such as sensitivity analysis, causal inference, and the social sciences.},
archivePrefix = {arXiv},
arxivId = {2010.09337},
author = {Molnar, Christoph and Casalicchio, Giuseppe and Bischl, Bernd},
doi = {10.1007/978-3-030-65965-3\_28},
eprint = {2010.09337},
isbn = {9783030659646},
issn = {18650937},
journal = {Communications in Computer and Information Science},
keywords = {Explainable artificial intelligence,Interpretable Machine Learning},
number = {01},
pages = {417--431},
title = {{Interpretable Machine Learning – A Brief History, State-of-the-Art and Challenges}},
volume = {1323},
year = {2020}
}



@article{HS2022,
abstract = {Tree-based models such as decision trees and random forests (RF) are a cornerstone of modern machine-learning practice. To mitigate overfitting, trees are typically regularized by a variety of techniques that modify their structure (e.g. pruning). We introduce Hierarchical Shrinkage (HS), a post-hoc algorithm that does not modify the tree structure, and instead regularizes the tree by shrinking the prediction over each node towards the sample means of its ancestors. The amount of shrinkage is controlled by a single regularization parameter and the number of data points in each ancestor. Since HS is a post-hoc method, it is extremely fast, compatible with any tree growing algorithm, and can be used synergistically with other regularization techniques. Extensive experiments over a wide variety of real-world datasets show that HS substantially increases the predictive performance of decision trees, even when used in conjunction with other regularization techniques. Moreover, we find that applying HS to each tree in an RF often improves accuracy, as well as its interpretability by simplifying and stabilizing its decision boundaries and SHAP values. We further explain the success of HS in improving prediction performance by showing its equivalence to ridge regression on a (supervised) basis constructed of decision stumps associated with the internal nodes of a tree. All code and models are released in a full-fledged package available on Github (github.com/csinva/imodels)},
archivePrefix = {arXiv},
arxivId = {2202.00858},
author = {Agarwal, Abhineet and Tan, Yan Shuo and Ronen, Omer and Singh, Chandan and Yu, Bin},
title = {{Hierarchical Shrinkage: improving the accuracy and interpretability of tree-based methods}},
url = {http://arxiv.org/abs/2202.00858},
  journal={arXiv preprint arXiv:2202.00858},
  year={2022}
}


@article{inTrees,
abstract = {Tree ensembles such as random forests and boosted trees are accurate but difficult to understand. In this work, we provide the interpretable trees (inTrees) framework that extracts, measures, prunes, selects, and summarizes rules from a tree ensemble, and calculates frequent variable interactions. The inTrees framework can be applied to multiple types of tree ensembles, e.g., random forests, regularized random forests, and boosted trees. We implemented the inTrees algorithms in the "inTrees" R package.},
author = {Deng, Houtao},
doi = {10.1007/s41060-018-0144-8},
journal = {International Journal of Data Science and Analytics},
keywords = {Boosted trees,Decision tree,Random forest,Rule extraction,Rule-based learner},
pages = {277--287},
title = {{Interpreting tree ensembles with inTrees}},
url = {https://doi.org/10.1007/s41060-018-0144-8},
volume = {7},
year = {2019}
}

@misc{Turkson2021,
author = {Turkson, Anthony Joe and Ayiah-Mensah, Francis and Nimoh, Vivian},
booktitle = {International Journal of Mathematics and Mathematical Sciences},
doi = {10.1155/2021/9307475},
issn = {16870425},
publisher = {Hindawi Limited},
title = {{Handling Censoring and Censored Data in Survival Analysis: A Standalone Systematic Literature Review}},
volume = {2021},
year = {2021}
}

@article{Tan2016,
archivePrefix = {arXiv},
arxivId = {1611.07115},
author = {Tan, Sarah and Soloviev, Matvey and Hooker, Giles and Wells, Martin T.},
eprint = {1611.07115},
number = {1},
title = {{Tree Space Prototypes: Another Look at Making Tree Ensembles Interpretable}},
url = {http://arxiv.org/abs/1611.07115},
year = {2016}
}


@article{Goldstein2015,
abstract = {This article presents individual conditional expectation (ICE) plots, a tool for visualizing the model estimated by any supervised learning algorithm. Classical partial dependence plots (PDPs) help visualize the average partial relationship between the predicted response and one or more features. In the presence of substantial interaction effects, the partial response relationship can be heterogeneous. Thus, an average curve, such as the PDP, can obfuscate the complexity of the modeled relationship. Accordingly, ICE plots refine the PDP by graphing the functional relationship between the predicted response and the feature for individual observations. Specifically, ICE plots highlight the variation in the fitted values across the range of a covariate, suggesting where and to what extent heterogeneities might exist. In addition to providing a plotting suite for exploratory analysis, we include a visual test for additive structure in the data-generating model. Through simulated examples and real datasets, we demonstrate how ICE plots can shed light on estimated models in ways PDPs cannot. Procedures outlined are available in the R package ICEbox.},
archivePrefix = {arXiv},
arxivId = {1309.6392},
author = {Goldstein, Alex and Kapelner, Adam and Bleich, Justin and Pitkin, Emil},
doi = {10.1080/10618600.2014.907095},
eprint = {1309.6392},
journal = {Journal of Computational and Graphical Statistics},
keywords = {Exploratory data analysis,Graphical method,Model visualization},
mendeley-groups = {selected Explainablity Techniques,About X-AI,Biblio for ECML-2022},
number = {1},
pages = {44--65},
title = {{Peeking Inside the Black Box: Visualizing Statistical Learning With Plots of Individual Conditional Expectation}},
volume = {24},
year = {2015}
}

@article{Friedman2001,
abstract = {Function estimation/approximation is viewed from the perspective of numerical optimization iti function space, rather than parameter space. A connection is made between stagewise additive expansions and steepest-descent minimization. A general gradient descent "boosting" paradigm is developed for additive expansions based on any fitting criterion. Specific algorithms are presented for least-squares, least absolute deviation, and Huber-M loss functions for regression, and multiclass logistic likelihood for classification. Special enhancements are derived for the particular case where the individual additive components are regression trees, and tools for interpreting such "TreeBoost" models are presented. Gradient boosting of regression trees produces competitives highly robust, interpretable procedures for both regression and classification, especially appropriate for mining less than clean data. Connections between this approach and the boosting methods of Freund and Shapire and Friedman, Hastie and Tibshirani are discussed.},
author = {Friedman, Jerome H.},
doi = {10.1214/aos/1013203451},
issn = {00905364},
journal = {Annals of Statistics},
keywords = {Boosting,Decision trees,Function estimation,Robust nonparametric regression},
mendeley-groups = {E-IRT paper references,Biblio for ECML-2022},
number = {5},
pages = {1189--1232},
title = {Greedy function approximation: A gradient boosting machine},
volume = {29},
year = {2001}
}

@article{Ribeiro2016,
abstract = {Despite widespread adoption, machine learning models remain mostly black boxes. Understanding the reasons behind predictions is, however, quite important in assessing trust, which is fundamental if one plans to take action based on a prediction, or when choosing whether to deploy a new model. Such understanding also provides insights into the model, which can be used to transform an untrustworthy model or prediction into a trustworthy one. In this work, we propose LIME, a novel explanation technique that explains the predictions of any classifier in an interpretable and faithful manner, by learning an interpretable model locally around the prediction. We also propose a method to explain models by presenting representative individual predictions and their explanations in a non-redundant way, framing the task as a submodular optimization problem. We demonstrate the flexibility of these methods by explaining different models for text (e.g. random forests) and image classification (e.g. neural networks). We show the utility of explanations via novel experiments, both simulated and with human subjects, on various scenarios that require trust: deciding if one should trust a prediction, choosing between models, improving an untrustworthy classifier, and identifying why a classifier should not be trusted.},
arxivId = {arXiv:1602.04938v3},
author = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
doi = {10.1145/2939672.2939778},
eprint = {arXiv:1602.04938v3},
isbn = {9781450342322},
journal = {Proceedings of the ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
mendeley-groups = {selected Explainablity Techniques,Biblio for ECML-2022},
pages = {1135--1144},
title = {"Why should i trust you?" Explaining the predictions of any classifier},
volume = {13-17-Augu},
year = {2016}
}


@article{Dedja2021,
author = {Dedja, Klest and Nakano, Felipe Kenji and Pliakos, Konstantinos and Vens, Celine},
journal = {ECML-PKDD , PharML Workshop, Bilbao, Spain (online).  Springer},
doi = {https://doi.org/10.1007/978-3-030-93733-1\_33},
keywords = {explainable ai, random forest,survival analysis},
mendeley-groups = {Biblio for ECML-2022},
pages = {1--8},
title = {{Explaining a Random Survival Forest by extracting prototype rules}},
year = {2021}
}


@article{Mead1992,
author = {Mead, A},
journal = {Journal of the Royal Statistical Society. Series D (The Statistician)},
mendeley-groups = {Biblio for ECML-2022,About X-AI},
number = {1},
pages = {27--39},
title = {{Review of the Development of Multidimensional Scaling Methods}},
volume = {41},
year = {1992}
}

@article{Pearson1901,
   author = {Karl Pearson},
   doi = {10.1080/14786440109462720},
   issn = {1941-5982},
   issue = {11},
   journal = {The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
   month = {11},
   pages = {559-572},
   publisher = {Informa UK Limited},
   title = {On lines and planes of closest fit to systems of points in space},
   volume = {2},
   url = {https://www-tandfonline-com.kuleuven.e-bronnen.be/doi/abs/10.1080/14786440109462720},
   year = {1901},
}

@inproceedings{vassilvitskii2006,
  title={k-means++: The advantages of careful seeding},
  author={Vassilvitskii, Sergei and Arthur, David},
  booktitle={Proceedings of the eighteenth annual ACM-SIAM symposium on Discrete algorithms},
  pages={1027--1035},
  year={2006}
}

@article{park2009,
  title={A simple and fast algorithm for K-medoids clustering},
  author={Park, Hae-Sang and Jun, Chi-Hyuck},
  journal={Expert systems with applications},
  volume={36},
  number={2},
  pages={3336--3341},
  year={2009},
  publisher={Elsevier}
}



@article{KaplanMeyer1958,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2281868},
 abstract = {In lifetesting, medical follow-up, and other fields the observation of the time of occurrence of the event of interest (called a death) may be prevented for some of the items of the sample by the previous occurrence of some other event (called a loss). Losses may be either accidental or controlled, the latter resulting from a decision to terminate certain observations. In either case it is usually assumed in this paper that the lifetime (age at death) is independent of the potential loss time; in practice this assumption deserves careful scrutiny. Despite the resulting incompleteness of the data, it is desired to estimate the proportion P(t) of items in the population whose lifetimes would exceed t (in the absence of such losses), without making any assumption about the form of the function P(t). The observation for each item of a suitable initial event, marking the beginning of its lifetime, is presupposed. For random samples of size N the product-limit (PL) estimate can be defined as follows: List and label the N observed lifetimes (whether to death or loss) in order of increasing magnitude, so that one has 0 ≤ t1' ≤ t2' ≤ ⋯ ≤ tN'. Then $\hat{P}(t) = \prod_r \lbrack(N - r)/(N - r + 1)\rbrack$, where r assumes those values for which tr' ≤ t and for which tr' measures the time to death. This estimate is the distribution, unrestricted as to form, which maximizes the likelihood of the observations. Other estimates that are discussed are the actuarial estimates (which are also products, but with the number of factors usually reduced by grouping); and reduced-sample (RS) estimates, which require that losses not be accidental, so that the limits of observation (potential loss times) are known even for those items whose deaths are observed. When no losses occur at ages less than t, the estimate of P(t) in all cases reduces to the usual binomial estimate, namely, the observed proportion of survivors.},
 author = {E. L. Kaplan and Paul Meier},
 journal = {Journal of the American Statistical Association},
 number = {282},
 pages = {457--481},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Nonparametric Estimation from Incomplete Observations},
 volume = {53},
 year = {1958}
}


@article{NodeHarvest,
   author = {N Meinshausen},
   issue = {4},
   journal = {The Annals of Applied Statistics},
   month = {12},
   pages = {2049-2072},
   title = {Node harvest},
   volume = {4},
   url = {https://www.jstor.org/stable/23362459},
   year = {2010},
}


@article{LionForest,
   author = {Ioannis Mollas and Nick Bassiliades and Grigorios Tsoumakas},
   doi = {10.1007/s10618-022-00839-y},
   journal = {Data Mining and Knowledge Discovery},
   keywords = {Explainable artificial intelligence,Interpretable machine learning,Local interpretation,Model-specific interpretation,Random forests},
   pages = {1521-1574},
   title = {Conclusive local interpretation rules for random forests},
   volume = {36},
   url = {https://doi.org/10.1007/s10618-022-00839-y},
   year = {2022},
}


@article{multilabel-LionForest,
   author = {Nikolaos Mylonas and Ioannis Mollas and Nick Bassiliades and Grigorios Tsoumakas},
   month = {7},
   title = {Local Multi-Label Explanations for Random Forest},
   journal={arXiv preprint arXiv:2207.01994},
   url = {https://arxiv.org/abs/2207.01994v1},
   year = {2022},
}



@article{MICE,
author = {Raghunathan, Trivellore and Lepkowski, James and Hoewyk, John and Solenberger, Peter},
year = {2000},
month = {11},
pages = {},
title = {A Multivariate Technique for Multiply Imputing Missing Values Using a Sequence of Regression Models},
volume = {27},
journal = {Survey Methodology}
}


@software{nhanes1997,
	title = {{NHANES} {III} plan and operations procedures manuals},
	url = {https://search.library.wisc.edu/catalog/999827443002121},
	publisher = {[Atlanta, Ga.?] : [National Centers for Disease Control and Prevention], [1997?]},
	author = {{National Health and Nutrition Examination Survey (U.S.)}},
	date = {1997}
}

@article{Ishwaran2008,
abstract = {We introduce random survival forests, a random forests method for the analysis of right-censored survival data. New survival splitting rules for growing survival trees are introduced, as is a new missing data algorithm for imputing missing data. A conservation-of-events principle for survival forests is introduced and used to define ensemble mortality, a simple interpretable measure of mortality that can be used as a predicted outcome. Several illustrative examples are given, including a case study of the prognostic implications of body mass for individuals with coronary artery disease. Computations for all examples were implemented using the freely available R-software package, random Survival Forest. {\textcopyright} Institute of Mathematical Statistics.},
archivePrefix = {arXiv},
arxivId = {arXiv:0811.1645v1},
author = {Ishwaran, Hemant and Kogalur, Udaya B. and Blackstone, Eugene H. and Lauer, Michael S.},
doi = {10.1214/08-AOAS169},
eprint = {arXiv:0811.1645v1},
issn = {19326157},
journal = {Annals of Applied Statistics},
keywords = {Conservation of events,Cumulative hazard function,Ensemble,Out-of-bag,Prediction error,Survival tree},
mendeley-groups = {Survival Analysis,Survival Analysis/Survival Forest and Trees},
number = {3},
pages = {841--860},
title = {{Random survival forests}},
volume = {2},
year = {2008}
}

@article{LeBlanc1993,
abstract = {A tree-based method for censored survival data is developed, based on maximizing the difference in survival between groups of patients represented by nodes in a binary tree. The method includes a pruning algorithm with optimal properties analogous to the classification and regression tree (CART) pruning algorithm. Uniform convergence of the estimates of the conditional cumulative hazard and survival functions is discussed, and an example is given to show the utility of the algorithm for developing prognostic classifications for patients. {\textcopyright} 1993 Taylor & Francis Group, LLC.},
author = {LeBlanc, Michael and Crowley, John},
doi = {10.1080/01621459.1993.10476296},
issn = {1537274X},
journal = {Journal of the American Statistical Association},
keywords = {Classification and regression tree,Regression trees,Survival analysis},
mendeley-groups = {Biblio for ECML-2022},
number = {422},
pages = {457--467},
title = {{Survival trees by goodness of split}},
volume = {88},
year = {1993}
}

@software{Breiman2002,
    title = {Software for the masses},
    publisher = {[Banff, Canada] : [Wald Lectures, Meeting of the Institute of Mathematical Statistics]},
    url = {http://www.stat.berkeley.edu/users/breiman},
    author = {Breiman, Leo},
    date = {2002}
}


@software{nhanes1997,
	title = {{NHANES} {III} plan and operations procedures manuals},
	url = {https://search.library.wisc.edu/catalog/999827443002121},
	publisher = {[Atlanta, Ga.?] : [National Centers for Disease Control and Prevention], [1997?]},
	author = {{National Health and Nutrition Examination Survey (U.S.)}},
	date = {1997}
}

@article{VanBuuren2007,
author = {Van Buuren, Stef},
doi = {10.1177/0962280206074463},
journal = {Statistical Methods in Medical Research},
mendeley-groups = {Biblio for ECML-2022},
month = {jun},
number = {3},
pages = {219--242},
title = {{Multiple imputation of discrete and continuous data by fully conditional specification}},
url = {www.scopus.com,},
volume = {16},
year = {2007}
}

@article{Vens2008,
abstract = {Hierarchical multi-label classification (HMC) is a variant of classification where instances may belong to multiple classes at the same time and these classes are organized in a hierarchy. This article presents several approaches to the induction of decision trees for HMC, as well as an empirical study of their use in functional genomics. We compare learning a single HMC tree (which makes predictions for all classes together) to two approaches that learn a set of regular classification trees (one for each class). The first approach defines an independent single-label classification task for each class (SC). Obviously, the hierarchy introduces dependencies between the classes. While they are ignored by the first approach, they are exploited by the second approach, named hierarchical single-label classification (HSC). Depending on the application at hand, the hierarchy of classes can be such that each class has at most one parent (tree structure) or such that classes may have multiple parents (DAG structure). The latter case has not been considered before and we show how the HMC and HSC approaches can be modified to support this setting. We compare the three approaches on 24 yeast data sets using as classification schemes MIPS's FunCat (tree structure) and the Gene Ontology (DAG structure). We show that HMC trees outperform HSC and SC trees along three dimensions: predictive accuracy, model size, and induction time. We conclude that HMC trees should definitely be considered in HMC tasks where interpretable models are desired. {\textcopyright} 2008 Springer Science+Business Media, LLC.},
author = {Vens, Celine and Struyf, Jan and Schietgat, Leander and D{\v{z}}eroski, Sa{\v{s}}o and Blockeel, Hendrik},
doi = {10.1007/s10994-008-5077-3},
issn = {08856125},
journal = {Machine Learning},
keywords = {Decision trees,Functional genomics,Hierarchical classification,Multi-label classification,Precision-recall analysis},
mendeley-groups = {Biblio for ECML-2022},
month = {nov},
number = {2},
pages = {185--214},
publisher = {Springer},
title = {{Decision trees for hierarchical multi-label classification}},
url = {https://link.springer.com/article/10.1007/s10994-008-5077-3},
volume = {73},
year = {2008}
}

@article{Wang2019,
abstract = {Survival analysis is a subfield of statistics where the goal is to analyze and model data where the outcome is the time until an event of interest occurs. One of the main challenges in this context is the presence of instances whose event outcomes become unobservable after a certain time point or when some instances do not experience any event during the monitoring period. This so-called censoring can be handled most effectively using survival analysis techniques. Traditionally, statistical approaches have been widely developed in the literature to overcome the issue of censoring. In addition, many machine learning algorithms have been adapted to deal with such censored data and tackle other challenging problems that arise in real-world data. In this survey, we provide a comprehensive and structured review of the statistical methods typically used and the machine learning techniques developed for survival analysis, along with a detailed taxonomy of the existing methods. We also discuss several topics that are closely related to survival analysis and describe several successful applications in a variety of real-world application domains. We hope that this article will give readers a more comprehensive understanding of recent advances in survival analysis and offer some guidelines for applying these approaches to solve new problems arising in applications involving censored data.},
archivePrefix = {arXiv},
arxivId = {1708.04649},
author = {Wang, Ping and Li, Yan and Reddy, Chandan K.},
doi = {10.1145/3214306},
eprint = {1708.04649},
issn = {15577341},
journal = {ACM Computing Surveys},
keywords = {Censoring,Concordance index,Cox model,Hazard rate,Machine learning,Regression,Survival analysis,Survival data},
mendeley-groups = {Survival Analysis,Biblio for ECML-2022},
number = {6},
pages = {1--39},
title = {{Machine learning for survival analysis: A survey}},
volume = {51},
year = {2019}
}

@article{Peto1972,
abstract = {Asymptotically efficient rank invariant test procedures for detecting differences between two groups of independent observations are derived. These are generalized to test between two groups of independent censored observations, to test between many groups of observations, and to test between groups after allowance for the effects of concomitant variables. One of these test procedures--the logrank--is particularly appropriate for comparing life tables, and can therefore be used in the analysis of clinical trials, industrial life-testing experiments and laboratory studies of animal carcinogenesis. It has greater local power than any other rank-invariant test procedure for detecting Lehmann-type differences between groups of independent observations subject to some right-censoring. The logrank test, although a rank test, can be presented in a format which exhibits the physical significance as well as the statistical significance of any important differences between groups of events.},
author = {Peto, Richard and Peto, Julian},
doi = {10.2307/2344317},
issn = {00359238},
journal = {Journal of the Royal Statistical Society. Series A (General)},
mendeley-groups = {Biblio for ECML-2022},
number = {2},
pages = {185},
publisher = {JSTOR},
title = {{Asymptotically Efficient Rank Invariant Test Procedures}},
url = {https://www.jstor.org/stable/10.2307/2344317?origin=crossref},
volume = {135},
year = {1972}
}

@misc{BostonDataControversy,
   title = {racist data destruction? A Boston housing dataset controversy},
   author ={Carlisle, M},
   publisher = {Medium},
   url = {https://medium.com/@docintangible/racist-data-destruction-113e3eff54a8},
   year = {2019},
   last-visited = {2022-10-12}
}


@misc{BostonDataset,
   title = {The Boston housing dataset},
   author ={Harrison, D. and Rubinfeld, D.L.},
   url  = {https://www.cs.toronto.edu/~delve/data/boston/bostonDetail.html},
   year = {1996},
   urldate = {2022-11-15}
}

%       %7E encodes the "~" in the environment

@misc{KDTree,
   title = {Nearest Neighbors},
   author ={scikit-learn developers},
   url = {https://scikit-learn.org/stable/modules/neighbors.html\#k-d-tree},
   last-visited = {2022-11-15},
   year = {2022}
}
%Vanderplas, J.

@misc{PCA,
   title = {Decomposing signals in components (matrix factorization problems)},
   author ={scikit-learn developers},
   url = {https://scikit-learn.org/stable/modules/decomposition.html\#pca},
   last-visited = {2022-11-15},
   year = {2022}
}

%https://scikit-learn.org/stable/modules/decomposition.html#pca


@book{Multi-event-SA,
   author = {Martin Crowder},
   isbn = {978-1-4398-7521-6},
   publisher = {CRC Press, Taylor and Francis Group},
   title = {Multivariate Survival Analysis and Competing Risks},
   year = {2012},
   address = {Boca Raton, USA},
}

@misc{river,
  title={River: machine learning for streaming data in Python},
  author={Montiel, Jacob and Halford, Max and Mastelini, Saulo Martiello
          and Bolmier, Geoffrey and Sourty, Raphael and Vaysse, Robin and Zouitine, Adil
          and Gomes, Heitor Murilo and Read, Jesse and Abdessalem, Talel and others},
  year={2021}
}

@article{Demsar2006,
abstract = {While methods for comparing two learning algorithms on a single data set have been scrutinized for quite some time already, the issue of statistical tests for comparisons of more algorithms on multiple data sets, which is even more essential to typical machine learning studies, has been all but ignored. This article reviews the current practice and then theoretically and empirically examines several suitable tests. Based on that, we recommend a set of simple, yet safe and robust non-parametric tests for statistical comparisons of classifiers: the Wilcoxon signed ranks test for comparison of two classifiers and the Friedman test with the corresponding post-hoc tests for comparison of more classifiers over multiple data sets. Results of the latter can also be neatly presented with the newly introduced CD (critical difference) diagrams.},
author = {Dem{\v{s}}ar, Janez},
issn = {15337928},
journal = {Journal of Machine Learning Research},
keywords = {Comparative studies,Friedman test,Multiple comparisons tests,Statistical methods,Wilcoxon signed ranks test},
mendeley-groups = {E-IRT paper references},
pages = {1--30},
title = {{Statistical comparisons of classifiers over multiple data sets}},
volume = {7},
year = {2006}
}


@article{cox1972,
title={Regression models and life-tables},
author={Cox, David R},
journal={Journal of the Royal Statistical Society: Series B (Methodological)},
volume={34},
number={2},
pages={187--202},
year={1972},
publisher={Wiley Online Library}
}

@article{Dzindolet2003,
abstract = {A recent and dramatic increase in the use of automation has not yielded comparable improvements in performance. Researchers have found human operators often underutilize (disuse) and overly rely on (misuse) automated aids (Parasuraman and Riley, 1997). Three studies were performed with Cameron University students to explore the relationship among automation reliability, trust, and reliance. With the assistance of an automated decision aid, participants viewed slides of Fort Sill terrain and indicated the presence or absence of a camouflaged soldier. Results from the three studies indicate that trust is an important factor in understanding automation reliance decisions. Participants initially considered the automated decision aid trustworthy and reliable. After observing the automated aid make errors, participants distrusted even reliable aids, unless an explanation was provided regarding why the aid might err. Knowing why the aid might err increased trust in the decision aid and increased automation reliance, even when the trust was unwarranted. Our studies suggest a need for future research focused on understanding automation use, examining individual differences in automation reliance, and developing valid and reliable self-report measures of trust in automation.},
author = {Dzindolet, Mary T. and Peterson, Scott A. and Pomranky, Regina A. and Pierce, Linda G. and Beck, Hall P.},
doi = {10.1016/S1071-5819(03)00038-7},
issn = {10715819},
journal = {International Journal of Human-Computer Studies},
keywords = {Automation reliance,Automation trust,Disuse,Misuse},
month = {jun},
number = {6},
pages = {697--718},
publisher = {Academic Press},
title = {{The role of trust in automation reliance}},
url = {https://linkinghub.elsevier.com/retrieve/pii/S1071581903000387},
volume = {58},
year = {2003}
}


@article{Cutillo2020,
  title={Machine intelligence in healthcare—perspectives on trustworthiness, explainability, usability, and transparency},
  author={Cutillo, Christine M and Sharma, Karlie R and Foschini, Luca and Kundu, Shinjini and Mackintosh, Maxine and Mandl, Kenneth D},
  journal={NPJ digital medicine},
  volume={3},
  number={1},
  pages={1--5},
  year={2020},
  publisher={Nature Publishing Group}
}


@article{Miller1956,
  title={The magical number seven, plus or minus two: Some limits on our capacity for processing information.},
  author={Miller, George A},
  journal={Psychological review},
  volume={63},
  number={2},
  pages={81},
  year={1956},
  publisher={American Psychological Association}
}


@article{Banerjee2012,
author = {Banerjee, Mousumi and Ding, Ying and Noone, Anne-Michelle},
doi = {10.1002/sim.4492},
issn = {02776715},
journal = {Statistics in Medicine},
keywords = {Bagging,Out-of-bag error,Random forest,Representative trees,Tree similarity metric},
mendeley-groups = {Biblio for ECML-2022},
month = {jul},
number = {15},
pages = {1601--1616},
publisher = {John Wiley & Sons, Ltd},
title = {{Identifying representative trees from ensembles}},
url = {https://onlinelibrary.wiley.com/doi/10.1002/sim.4492},
volume = {31},
year = {2012}
}


@article{Kocev2013,
abstract = {In this paper, we address the task of learning models for predicting structured outputs. We consider both global and local predictions of structured outputs, the former based on a single model that predicts the entire output structure and the latter based on a collection of models, each predicting a component of the output structure. We use ensemble methods and apply them in the context of predicting structured outputs. We propose to build ensemble models consisting of predictive clustering trees, which generalize classification trees: these have been used for predicting different types of structured outputs, both locally and globally. More specifically, we develop methods for learning two types of ensembles (bagging and random forests) of predictive clustering trees for global and local predictions of different types of structured outputs. The types of outputs considered correspond to different predictive modeling tasks: multi-target regression, multi-target classification, and hierarchical multi-label classification. Each of the combinations can be applied both in the context of global prediction (producing a single ensemble) or local prediction (producing a collection of ensembles). We conduct an extensive experimental evaluation across a range of benchmark datasets for each of the three types of structured outputs. We compare ensembles for global and local prediction, as well as single trees for global prediction and tree collections for local prediction, both in terms of predictive performance and in terms of efficiency (running times and model complexity). The results show that both global and local tree ensembles perform better than the single model counterparts in terms of predictive power. Global and local tree ensembles perform equally well, with global ensembles being more efficient and producing smaller models, as well as needing fewer trees in the ensemble to achieve the maximal performance. {\textcopyright} 2012 Elsevier Ltd.},
author = {Kocev, Dragi and Vens, Celine and Struyf, Jan and D{\v{z}}eroski, Sa{\v{s}}o},
doi = {10.1016/j.patcog.2012.09.023},
issn = {00313203},
journal = {Pattern Recognition},
keywords = {Ensemble methods,Hierarchical multi-label classification,Multi-target classification,Multi-target regression,Predictive clustering trees,Structured outputs},
mendeley-groups = {Biblio for ECML-2022},
month = {mar},
number = {3},
pages = {817--833},
publisher = {Pergamon},
title = {{Tree ensembles for predicting structured outputs}},
volume = {46},
year = {2013}
}


@article{Breiman2001,
author = {Breiman, Leo},
doi = {10.1023/A:1010933404324},
issn = {08856125},
journal = {Machine Learning},
keywords = {Classification,Ensemble,Regression},
mendeley-groups = {Biblio for ECML-2022},
month = {oct},
number = {1},
pages = {5--32},
publisher = {Springer},
title = {{Random forests}},
url = {https://link.springer.com/article/10.1023/A:1010933404324},
volume = {45},
year = {2001}
}



@article{Lundberg2017,
abstract = {Understanding why a model makes a certain prediction can be as crucial as the prediction's accuracy in many applications. However, the highest accuracy for large modern datasets is often achieved by complex models that even experts struggle to interpret, such as ensemble or deep learning models, creating a tension between accuracy and interpretability. In response, various methods have recently been proposed to help users interpret the predictions of complex models, but it is often unclear how these methods are related and when one method is preferable over another. To address this problem, we present a unified framework for interpreting predictions, SHAP (SHapley Additive exPlanations). SHAP assigns each feature an importance value for a particular prediction. Its novel components include: (1) the identification of a new class of additive feature importance measures, and (2) theoretical results showing there is a unique solution in this class with a set of desirable properties. The new class unifies six existing methods, notable because several recent methods in the class lack the proposed desirable properties. Based on insights from this unification, we present new methods that show improved computational performance and/or better consistency with human intuition than previous approaches.},
archivePrefix = {arXiv},
arxivId = {1705.07874},
author = {Lundberg, Scott M. and Lee, Su In},
eprint = {1705.07874},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
mendeley-groups = {Biblio for ECML-2022},
number = {Section 2},
pages = {4766--4775},
title = {{A unified approach to interpreting model predictions}},
volume = {2017-Decem},
year = {2017}
}

@article{Benard2021,
archivePrefix = {arXiv},
arxivId = {1908.06852},
author = {B{\'{e}}nard, Cl{\'{e}}ment and Biau, G{\'{e}}rard and {Da Veiga}, S{\'{e}}bastien and Scornet, Erwan},
doi = {10.1214/20-EJS1792},
eprint = {1908.06852},
issn = {19357524},
journal = {Electronic Journal of Statistics},
keywords = {Classification,Interpretability,Random forests,Rules,Stability},
mendeley-groups = {About X-AI,Biblio for ECML-2022},
number = {1},
pages = {427--505},
title = {{Sirus: Stable and interpretable rule set for classification}},
volume = {15},
year = {2021}
}

@article{Aria2021,
abstract = {The growing success of Machine Learning (ML) is making significant improvements to predictive models, facilitating their integration in various application fields. Despite its growing success, there are some limitations and disadvantages: the most significant is the lack of interpretability that does not allow users to understand how particular decisions are made. Our study focus on one of the best performing and most used models in the Machine Learning framework, the Random Forest model. It is known as an efficient model of ensemble learning, as it ensures high predictive precision, flexibility, and immediacy; it is recognized as an intuitive and understandable approach to the construction process, but it is also considered a Black Box model due to the large number of deep decision trees produced within it. The aim of this research is twofold. We present a survey about interpretative proposal for Random Forest and then we perform a machine learning experiment providing a comparison between two methodologies, inTrees, and NodeHarvest, that represent the main approaches in the rule extraction framework. The proposed experiment compares methods performance on six real datasets covering different data characteristics: n. of observations, balanced/unbalanced response, the presence of categorical and numerical predictors. This study contributes to picture a review of the methods and tools proposed for ensemble tree interpretation, and identify, in the class of rule extraction approaches, the best proposal.},
author = {Aria, Massimo and Cuccurullo, Corrado and Gnasso, Agostino},
doi = {10.1016/j.mlwa.2021.100094},
issn = {26668270},
journal = {Machine Learning with Applications},
mendeley-groups = {Biblio for ECML-2022,About X-AI},
number = {January},
pages = {100094},
publisher = {Elsevier Ltd.},
title = {{A comparison among interpretative proposals for Random Forests}},
url = {https://doi.org/10.1016/j.mlwa.2021.100094},
volume = {6},
year = {2021}
}

@article{Tan2020,
archivePrefix = {arXiv},
arxivId = {1611.07115},
author = {Tan, Sarah and Soloviev, Matvey and Hooker, Giles and Wells, Martin T.},
doi = {10.1145/3412815.3416893},
eprint = {1611.07115},
isbn = {9781450381031},
journal = {FODS 2020 - Proceedings of the 2020 ACM-IMS Foundations of Data Science Conference},
keywords = {interpretability,prototypes,tree ensemble classifiers},
mendeley-groups = {Biblio for ECML-2022},
pages = {23--34},
title = {{Tree Space Prototypes: Another Look at Making Tree Ensembles Interpretable}},
year = {2020}
}


@article{Wang2009,
abstract = {With the effectiveness of therapeutic agents ever decreasing and the increased incidence of multi-drug resistant pathogens, there is a clear need for administration of more potent, potentially more toxic, drugs. Alternatively, biopharmaceuticals may hold potential but require specialised protection from premature in vivo degradation. Thus, a paralleled need for specialised drug delivery systems has arisen. Although cell-mediated drug delivery is not a completely novel concept, the few applications described to date are not yet ready for in vivo application, for various reasons such as drug-induced carrier cell death, limited control over the site and timing of drug release and/or drug degradation by the host immune system. Here, we present our hypothesis for a new drug delivery system, which aims to negate these limitations. We propose transport of nanoparticle-encapsulated drugs inside autologous macrophages polarised to M1 phenotype for high mobility and treated to induce transient phagosome maturation arrest. In addition, we propose a significant shift of existing paradigms in the study of host-microbe interactions, in order to study microbial host immune evasion and dissemination patterns for their therapeutic utilisation in the context of drug delivery. We describe a system in which microbial strategies may be adopted to facilitate absolute control over drug delivery, and without sacrificing the host carrier cells. We provide a comprehensive summary of the lessons we can learn from microbes in the context of drug delivery and discuss their feasibility for in vivo therapeutic application. We then describe our proposed “synthetic microbe drug delivery system” in detail. In our opinion, this multidisciplinary approach may hold the solution to effective, controlled drug delivery.},
author = {Wang, Minghui and Zhang, Heping},
doi = {10.4310/sii.2009.v2.n3.a11},
issn = {19387989},
journal = {Statistics and Its Interface},
keywords = {Random forest, Classification, Smallest forest,,and phrases,classification,random forest},
mendeley-groups = {About X-AI,Biblio for ECML-2022},
number = {3},
pages = {381--388},
title = {{Search for the smallest random forest}},
volume = {2},
year = {2009}
}


@article{Biclustering,
  title={Network inference with ensembles of bi-clustering trees},
  author={Pliakos, Konstantinos and Vens, Celine},
  journal={BMC bioinformatics},
  volume={20},
  number={1},
  pages={1--12},
  year={2019},
  publisher={Springer}
}


@article{Mollas2019,
abstract = {Towards a future where machine learning systems will integrate into every aspect of people's lives, researching methods to interpret such systems is necessary, instead of focusing exclusively on enhancing their performance. Enriching the trust between these systems and people will accelerate this integration process. Many medical and retail banking/finance applications use state-of-the-art machine learning techniques to predict certain aspects of new instances. Tree ensembles, like random forests, are widely acceptable solutions on these tasks, while at the same time they are avoided due to their black-box uninterpretable nature, creating an unreasonable paradox. In this paper, we provide a sequence of actions for shedding light on the predictions of the misjudged family of tree ensemble algorithms. Using classic unsupervised learning techniques and an enhanced similarity metric, to wander among transparent trees inside a forest following breadcrumbs, the interpretable essence of tree ensembles arises. An explanation provided by these systems using our approach, which we call "LionForests", can be a simple, comprehensive rule.},
archivePrefix = {arXiv},
arxivId = {1911.08780},
author = {Mollas, Ioannis and Tsoumakas, Grigorios and Bassiliades, Nick},
eprint = {1911.08780},
pages = {1--8},
title = {{LionForests: Local Interpretation of Random Forests through Path Selection}},
url = {http://arxiv.org/abs/1911.08780},
year = {2019}
}
@article{Zhou2016,
abstract = {We propose a procedure to build a decision tree which approximates the performance of complex machine learning models. This single approximation tree can be used to interpret and simplify the predicting pattern of random forests (RFs) and other models. The use of a tree structure is particularly relevant in medical questionnaires where it enables an adaptive shortening of the questionnaire, reducing response burden. We study the asymptotic behavior of splits and introduce an improved splitting method designed to stabilize tree structure. Empirical studies on both simulation and real data sets illustrate that our method can simultaneously achieve high approximation power and stability.},
title={Interpreting models via single tree approximation},
author={Zhou, Yichen and Hooker, Giles},
journal={arXiv preprint arXiv:1610.09036},
year={2016}
}


@article{Moore2018,
abstract = {Every day more technologies and services are backed by complex machine-learned models, consuming large amounts of data to provide a myriad of useful services. While users are willing to provide personal data to enable these services, their trust in and engagement with the systems could be improved by providing insight into how the machine learned decisions were made. Complex ML systems are highly effective but many of them are black boxes and give no insight into how they make the choices they make. Moreover, those that do often do so at the model-level rather than the instance-level. In this work we present a method for deriving explanations for instance-level decisions in tree ensembles. As this family of models accounts for a large portion of industrial machine learning, this work opens up the possibility for transparent models at scale.},
annote = {IDEA: finding (maximal) intervals of influence of variables within the RF},
author = {Moore, Alexander and Murdock, Vanessa and Cai, Yaxiong and Jones, Kristine},
doi = {10.1145/3209978.3210151},
isbn = {9781450356572},
journal = {41st International ACM SIGIR Conference on Research and Development in Information Retrieval, SIGIR 2018},
keywords = {Boosted trees,Model explainability,Transparent ir},
pages = {1241--1244},
title = {{Transparent tree ensembles}},
year = {2018}
}

@article{Zhao2019,
title={iForest: Interpreting random forests via visual analytics},
doi = {10.1109/TVCG.2018.2864475},
issn = {19410506},
author={Zhao, Xun and Wu, Yanhong and Lee, Dik Lun and Cui, Weiwei},
journal={IEEE Transactions on Visualization and Computer Graphics},
keywords = {Interpretable Machine Learning,Random Forest Visualization,Random Forests,Visual Analytics},
publisher={IEEE},
volume={25},
number={1},
pages={407--416},
year={2019},
}

@article{hinton2002,
  title={Stochastic neighbor embedding},
  author={Hinton, Geoffrey E and Roweis, Sam},
  journal={Advances in neural information processing systems},
  volume={15},
  year={2002}
}

@article{Hara2018,
abstract = {Tree ensembles, such as random forests, are renowned for their high prediction performance. However, their interpretability is critically limited due to the enormous complexity. In this study, we propose a method to make a complex tree ensemble inter-pretable by simplifying the model. Specifically , we formalize the simplification of tree ensembles as a model selection problem. Given a complex tree ensemble, we aim at obtaining the simplest representation that is essentially equivalent to the original one. To this end, we derive a Bayesian model selection algorithm that optimizes the simplified model while maintaining the prediction performance. Our numerical experiments on several datasets showed that complicated tree ensembles were approximated interpretably.},
author = {Hara, Satoshi},
journal = {International Conference on Artificial Intelligence and Statistics, AISTATS 2018},
title = {{Making Tree Ensembles Interpretable : A Bayesian Model Selection Approach}},
volume = {84},
year = {2018}
}

@article{Chipman1998,
author = {Chipman, Hugh A and George, Edward I and Mcculloch, Robert E},
journal={Computing Science and Statistics},
keywords = {added tree plot,bayes,clustering,mcmc,multidimensional scaling,stochastic search,tree metrics},
title = {{Making sense of a Forest of trees}},
pages={84--92},
year = {1998}
}

